Dwarf Galaxy Integral-field Survey (DGIS): survey overview and the result of global mass-metallicity relation

Low-mass galaxies are the building blocks of massive galaxies in the framework of hierarchical structure formation. To enable detailed studies of galactic ecosystems in dwarf galaxies by spatially resolving different galactic components, we have carried out the Dwarf Galaxy Integral-field Survey (DGIS). This survey aims to acquire observations with spatial resolutions as high as 10 to 100 pc while maintaining reasonably high signal-to-noise ratios with VLT/MUSE and ANU-2.3m/WiFeS. The whole sample will be composed of 65 dwarf galaxies with $M_{\rm \ast}$ $<$ 10$^{9}$ $\rm M_{\odot}$, selected from the Spitzer Local Volume Legacy Survey. The overall scientific goals include studying baryonic cycles in dwarf galaxies, searching for off-nuclear (intermediate)-massive black holes, and quantifying the inner density profiles of dark matter. In this work, we describe the sample selection, data reduction, and high-level data products. By integrating the spectra over the field of view for each galaxy, we obtained the integrated gas-phase metallicity and discussed its dependence on stellar mass and SFR. We find that the overall relation between metallicity and stellar mass of our DGIS nearly follows the extrapolation from the higher mass end. Its dispersion does not decrease by invoking the dependence on SFR.

==> ulem/README <==

  The ulem package provides various types of underlining that can stretch
  between words and be broken across lines in LaTeX or plain TeX.
  In LaTeX ulem replaces italics with underlining in \em-phasized text.
  A declaration of \normalem (or the \usepackage option "normalem") restores 
  the normal \em and \emph behavior.

  Copyright 1989-2019 by Donald Arseneau (Vancouver, Canada; asnd@triumf.ca)

  This software may be freely transmitted, reproduced, or modified for any
  purpose provided that this copyright notice is left intact.  

